Deep Underground Neutrino Experiment (DUNE), Far Detector Technical Design Report, Volume II: DUNE Physics

The preponderance of matter over antimatter in the early universe, the dynamics of the supernovae that produced the heavy elements necessary for life, and whether protons eventually decay -- these mysteries at the forefront of particle physics and astrophysics are key to understanding the early evolution of our universe, its current state, and its eventual fate. DUNE is an international world-class experiment dedicated to addressing these questions as it searches for leptonic charge-parity symmetry violation, stands ready to capture supernova neutrino bursts, and seeks to observe nucleon decay as a signature of a grand unified theory underlying the standard model. The DUNE far detector technical design report (TDR) describes the DUNE physics program and the technical designs of the single- and dual-phase DUNE liquid argon TPC far detector modules. Volume II of this TDR, DUNE Physics, describes the array of identified scientific opportunities and key goals. Crucially, we also report our best current understanding of the capability of DUNE to realize these goals, along with the detailed arguments and investigations on which this understanding is based. This TDR volume documents the scientific basis underlying the conception and design of the LBNF/DUNE experimental configurations. As a result, the description of DUNE's experimental capabilities constitutes the bulk of the document. Key linkages between requirements for successful execution of the physics program and primary specifications of the experimental configurations are drawn and summarized. This document also serves a wider purpose as a statement on the scientific potential of DUNE as a central component within a global program of frontier theoretical and experimental particle physics research. Thus, the presentation also aims to serve as a resource for the particle physics community at large.

==> generated/reqdefs-DP-CALIB.tex <==
% This file is generated, any edits may be lost.

% It defines macros which expand to corresponding
% specification values for subsystem DP-CALIB


\def\dpdatavolumelaser{$>\,\SI{37}{TB/yr/10 kt}$}
\def\dpdatavolumepns{$>\,\SI{170}{TB/yr/10 kt}$}
\def\dpefieldcalibcoverage{$>\,\SI{93}{\%}$}
\def\dpefieldcalibgranularity{\SI{10 x 10 x 10}{\centi\metre}}
\def\dpefieldcalibprecision{\SI{1}{\%}}
\def\dplaserpositionprecision{\SI{0.5}{\milli\radian}}
\def\dpneutronsourcecoverage{$>\,\SI{75}{\%}$}


==> generated/reqdefs-DP-CISC.tex <==
% This file is generated, any edits may be lost.

% It defines macros which expand to corresponding
% specification values for subsystem DP-CISC


\def\dpcameracoldcoverage{$>\,$80\% of HV surfaces}
\def\dpeleclifetimeprec{$<\,$2.3\%}
\def\dpeleclifetimerange{\SIrange{0.04}{10}{ms} in cryostat, \SIrange{0.04}{30}{ms} inline}
\def\dpinstefield{$<\,\SI{30}{kV/cm}$}
\def\dpinstnoise{$<<\,\SI{1000}\,e^- $}
\def\dpslowcontrolalarmrate{$<\,$150/day}
\def\dpslowcontrolarchiverate{\SI{0.02}{Hz}}
\def\dpslowcontrolnumvars{$>\,\num{150000}$}
\def\dptemprepro{$<\,\SI{5}{mK}$}
\def\dptempstability{$<\,\SI{2}{mK}$ at all places and times}


==> generated/reqdefs-DP-CRP.tex <==
% This file is generated, any edits may be lost.

% It defines macros which expand to corresponding
% specification values for subsystem DP-CRP


\def\dpcrpvertprecision{$<\,\SI{1}{\milli\meter}$}


==> generated/reqdefs-DP-DAQ.tex <==
% This file is generated, any edits may be lost.

% It defines macros which expand to corresponding
% specification values for subsystem DP-DAQ


\def\dpdaqdeadtime{}
\def\dpDAQreadout{\SI{65}{GB/s} per dual phase detector module}
\def\dpDAQreadoutwindow{\SI{10}{\micro\second} < readout window < \SI{100}{s}}
\def\dpDAQthroughput{\SI{2}{GB/s} average storage throughput; \SI{100}{GB/s} peak temporary storage throughput per dual phase detector module}
\def\dpdatarecord{}
\def\dpdataverification{}
\def\dptriggercalibration{}
\def\dptriggerhighenergy{$>\,$\SI{100}{\MeV}}
\def\dptriggerlowenergy{$>\,$\SI{10}{\MeV}}


==> generated/reqdefs-DP-ELEC.tex <==
% This file is generated, any edits may be lost.

% It defines macros which expand to corresponding
% specification values for subsystem DP-ELEC




==> generated/reqdefs-DP-FD.tex <==
% This file is generated, any edits may be lost.

% It defines macros which expand to corresponding
% specification values for subsystem DP-FD


\def\dp{}
\def\dpdenonfenoise{$<<\,\SI{1000}\,e^- $}
\def\dpdpadcnumberofbits{\num{12} bits}
\def\dpdpadcsamplingfreq{$\sim\,\SI{2.5}{\mega\hertz}$}
\def\dpdpcathoderesistivity{$>\,\SI{1}{\mega\ohm/square}$}
\def\dpdpcepowerconsumption{$<\,\SI{50}{ mW/channel} $}
\def\dpdpcrpeffgain{\num{6}}
\def\dpdpcrpgaps{$<\,\SI{30}{mm}$ between adjacent CRPs}
\def\dpdpcrpplanarity{$\pm\,\SI{0.5}{mm}$}
\def\dpdpcrpstripspacing{$<\,\SI{4.7}{mm}$}
\def\dpdpcryomonitordevices{}
\def\dpdpdataratetotape{$<\,\SI{30}{PB/year}$}
\def\dpdpdeadchannels{$<\,\SI{1}{\%}$}
\def\dpdpdetmoduptime{$>\,$90\%}
\def\dpdpdetuptime{$>\,$98\%}
\def\dpdpfepeaktime{\SI{1}{\micro\second}}
\def\dpdphvpsripple{$<\,\SI{100}e^-$}
\def\dpdphvsfielduniformity{$<\,\SI{1}{\%}$ throughout volume}
\def\dpdplarimpuritycontrib{$<<\,\SI{30}{ppt} $}
\def\dpdplarncontamination{$<\,\SI{3}{ppm}$}
\def\dpdplarpurity{$>$\,\SI{5}{ms}}
\def\dpdplightyield{$>\,\SI{1}{PE/MeV}$ (at anode), $>\,\SI{5}{PE/MeV}$ (avg  over active volume)}
\def\dpdplocalefields{$<\,\SI{30}{kV/cm}$}
\def\dpdpmindriftfield{$>$\,\SI{250}{ V/cm}}
\def\dpdpmisalignmentfielduniformity{$<\,1\,$\% throughout volume}
\def\dpdpradiopurity{less than that from $^{39}$Ar}
\def\dpdpsignalsaturation{\num{7500000} electrons}
\def\dpdpsntrigger{$>\,\SI{95}{\%}$ efficiency for a SNB producing at least 60 interactions with a neutrino energy >10 MeV in 12 kt of active detector mass during the first 10 seconds of the burst.}
\def\dpdpsystemnoise{$<\,\SI{1000}\,e^-$}
\def\dpdptimeresolutionpds{$<\,\SI{1}{\micro\second}$}


==> generated/reqdefs-DP-HV.tex <==
% This file is generated, any edits may be lost.

% It defines macros which expand to corresponding
% specification values for subsystem DP-HV


\def\dphvdbredundancy{$>\,\num{2}$ HVDB chain}


==> generated/reqdefs-DP-INST.tex <==
% This file is generated, any edits may be lost.

% It defines macros which expand to corresponding
% specification values for subsystem DP-INST


\def\dpcleanroomspecs{>ISO-8}
\def\dpcoldboxcryo{Independent operation of the four cold boxes}
\def\dphandlingspecs{Fulfill material handling specification}
\def\dpmaterialbuffer{>1 month}
\def\dpundergroundstorage{>4~\dshorts{crp}}


==> generated/reqdefs-DP-PDS.tex <==
% This file is generated, any edits may be lost.

% It defines macros which expand to corresponding
% specification values for subsystem DP-PDS


\def\dphitrelativetiming{$<\,\SI{100}{ns RMS}$}
\def\dphitsnr{$>\,\num{5}$}
\def\dppdsanalogrange{$>\,\SI{100}{PE/(ch\times 6\nano\second)}$}
\def\dppmtdarkrate{$<\,\SI{100}{kHz}$}


==> generated/reqdefs-SP-APA.tex <==
% This file is generated, any edits may be lost.

% It defines macros which expand to corresponding
% specification values for subsystem SP-APA


\def\spapaactivearea{Maximize total active area.}
\def\spapabadchannels{$<$1\%, with a goal of $<$0.5\%}
\def\spapabiasvoltage{The setup, including boards, must hold 150\% of max operating voltage.}
\def\spapaframeplanarity{$<$\SI{5}{mm}}
\def\spapaunitsize{\SI{6.0}{m} tall $\times$ \SI{2.3}{m} wide}
\def\spapawiretension{\SI{6}{N} $\pm$ \SI{1}{N}}


==> generated/reqdefs-SP-CALIB.tex <==
% This file is generated, any edits may be lost.

% It defines macros which expand to corresponding
% specification values for subsystem SP-CALIB


\def\spdatavolumelaser{$>\SI{184}{TB/yr/10 kt}$}
\def\spdatavolumepns{$>\SI{144}{TB/yr/10 kt}$}
\def\spefieldcalibcoverage{$>\SI{75}{\%}$}
\def\spefieldcalibgranularity{$~30\times 30\times 30~$\SI{}{\centi\metre\cubed}}
\def\spefieldcalibprecision{$\SI{1}{\%}$}
\def\splaserlocationprecision{$~\SI{0.5}{\milli\radian}$}
\def\spneutronsourcecoverage{$>\SI{75}{\%}$}


==> generated/reqdefs-SP-CISC.tex <==
% This file is generated, any edits may be lost.

% It defines macros which expand to corresponding
% specification values for subsystem SP-CISC


\def\spcameracoldcoverage{$>\,$80\% of HV surfaces}
\def\speleclifetimeprec{$<\,$1.4\%}
\def\speleclifetimerange{\SIrange{0.04}{10}{ms} in cryostat, \SIrange{0.04}{30}{ms} inline}
\def\spinstefield{$<\,\SI{30}{kV/cm}$}
\def\spinstnoise{$<<\,\SI{1000}\,e^- $}
\def\spslowcontrolalarmrate{$<\,$150/day}
\def\spslowcontrolarchiverate{\SI{0.02}{Hz}}
\def\spslowcontrolnumvars{$>\,\num{150000}$}
\def\sptemprepro{$<\,\SI{5}{mK}$}
\def\sptempstability{$<\,\SI{2}{mK}$ at all places and times}


==> generated/reqdefs-SP-DAQ.tex <==
% This file is generated, any edits may be lost.

% It defines macros which expand to corresponding
% specification values for subsystem SP-DAQ


\def\spdaqdeadtime{}
\def\spDAQreadout{1.5 TB/s per single phase detector module}
\def\spDAQreadoutwindow{10 $\mu$s < readout window < 100 s}
\def\spDAQthroughput{10 Gb/s average storage throughput; 100 Gb/s peak temporary storage throughput per single phase detector module}
\def\spdatarecord{}
\def\spdataverification{}
\def\sptriggercalibration{}
\def\sptriggerhighenergy{$>$\SI{100}{\MeV}}
\def\sptriggerlowenergy{$>$\SI{10}{\MeV}}


==> generated/reqdefs-SP-ELEC.tex <==
% This file is generated, any edits may be lost.

% It defines macros which expand to corresponding
% specification values for subsystem SP-ELEC


\def\spcoldcablesxsec{\SI{6.35}{cm} (2.5")}
\def\spFEMBdatalink{\num{4} at \SI{1.28}{Gbps}}
\def\spgainFEamplifier{$\sim\SI{20}{mV/fC}$}
\def\spnumchannelsFEMB{\num{128}}
\def\spnumFEbaselines{\num{2}}
\def\spnumberFEMBperWIB{\num{4}}
\def\spsyncronizationCE{\SI{50}{ns}}
\def\spWIBdatalink{\SI{10}{Gbps}}


==> generated/reqdefs-SP-FD.tex <==
% This file is generated, any edits may be lost.

% It defines macros which expand to corresponding
% specification values for subsystem SP-FD


\def\sp{}
\def\spadcnumberofbits{\num{12} bits}
\def\spadcsamplingfreq{$\sim\,\SI{2}{\mega\hertz}$}
\def\spapagaps{$<\,\SI{15}{mm}$ between APAs on same support beam; $<\,\SI{30}{mm}$ between APAs on different support beams}
\def\spapawireangles{\SI{0}{\degree} for collection wires, $\pm\,$\SI{35.7}{\degree} for induction wires}
\def\spapawirepostolerance{$\pm\,\SI{0.5}{mm}$}
\def\spapawirespacing{\SI{4.669}{mm} for U,V; \SI{4.790}{mm} for X,G}
\def\spcathoderesistivity{$>\,\SI{1}{\mega\ohm/square}$}
\def\spcepowerconsumption{$<\,\SI{50}{ mW/channel} $}
\def\spcryomonitordevices{}
\def\spdataratetotape{$<\,\SI{30}{PB/year}$}
\def\spdeadchannels{$<\,\SI{1}{\%}$}
\def\spdpdetmoduptime{$>\,$90\%}
\def\spdpdetuptime{$>\,$98\%}
\def\spfepeaktime{\SI{1}{\micro\second}}
\def\sphvpsripple{$<\,\SI{100}e^-$}
\def\sphvsfielduniformity{$<\,\SI{1}{\%}$ throughout volume}
\def\splarimpuritycontrib{$<<\,\SI{30}{ppt} $}
\def\splarncontamination{$<\,\SI{25}{ppm}$}
\def\splarpurity{$<$\,\SI{100}{ppt}}
\def\splightyield{$>\,\SI{20}{PE/MeV}$ (avg), $>\,\SI{0.5}{PE/MeV}$ (min)}
\def\splocalefields{$<\,\SI{30}{kV/cm}$}
\def\spmindriftfield{$>$\,\SI{250}{ V/cm}}
\def\spmisalignmentfielduniformity{$<\,1\,$\% throughout volume}
\def\spnonfenoise{$<<\,\SI{1000}\,e^- $}
\def\spradiopurity{less than that from $^{39}$Ar}
\def\spsntrigger{$>\,\SI{95}{\%}$ efficiency for a SNB producing at least 60 interactions with a neutrino energy >10 MeV in 12 kt of active detector mass during the first 10 seconds of the burst.}
\def\spspsignalsaturation{\num{500000} $e^-$}
\def\spsystemnoise{$<\,\SI{1000}\,e^-$}
\def\sptimeresolutionpds{$<\,\SI{1}{\micro\second}$}


==> generated/reqdefs-SP-HV.tex <==
% This file is generated, any edits may be lost.

% It defines macros which expand to corresponding
% specification values for subsystem SP-HV


\def\sphvconnectionredundancy{Two-fold}
\def\sppowersupplystability{$>\,\SI{95}{\%}$ uptime}


==> generated/reqdefs-SP-INST.tex <==
% This file is generated, any edits may be lost.

% It defines macros which expand to corresponding
% specification values for subsystem SP-INST


\def\spapastoragesd{700 m$^2$}
\def\spcleanroomspecification{ISO 8}
\def\spcleanroomuvfilters{filter $<\SI{400}{nm}$ for $>$ 2 wk exp; $<\SI{520}{nm}$ all else}
\def\splogisticsmaterialhandling{SURF Material Handling Specification}
\def\splogisticsmaterialsbuffer{$>1$ month}
\def\splogisticsshippingcoord{2 wk notice to CMGC}


==> generated/reqdefs-SP-PDS.tex <==
% This file is generated, any edits may be lost.

% It defines macros which expand to corresponding
% specification values for subsystem SP-PDS


\def\spapainstall{$>\,\SI{1}{\milli\meter}$}
\def\spenvhumiditylimit{$<\,\SI{50}{\%}$ RH at \SI{70}{\degree F}}
\def\spenvlightexposure{No exposure to sunlight. All other unfiltered sources: $<\,\num{30}$ minutes integrated across all exposures}
\def\splighttightness{Cryostat light leaks responsible for $<\,\SI{10}{\%}$  of data transferred from PDS to DAQ}
\def\spmechcompatibility{$>\,\SI{1}{\milli\meter}$}
\def\spmechdeflection{$<\,\SI{5}{\milli\meter}$}
\def\sppdscable{$<\,\SI{6}{\milli\meter}$}
\def\sppdscablemate{\SI{0}{\milli\meter} separation mechanically allowed}
\def\sppdscleanroomassbly{Class \num{100000} clean assembly area}
\def\sppdsclearance{$>\,\SI{0.5}{\milli\meter}$}
\def\sppdsdarkrate{$<\,\SI{1}{kHz}$}
\def\sppdsdatarate{$<\,\SI{8}{Gbps}$}
\def\sppdsdynamicrange{$<\,\SI{20}{\%}$}
\def\sppdssignaltonoise{$>\,\num{4}$}
\def\spspatiallocalization{$<\,\SI{2.5}{\meter}$}


==> generated/reqdefs.tex <==
% generated file, do not edit\input{generated/reqdefs-SP-FD}
\input{generated/reqdefs-DP-FD}
\input{generated/reqdefs-SP-APA}
\input{generated/reqdefs-DP-CRP}
\input{generated/reqdefs-SP-HV}
\input{generated/reqdefs-DP-HV}
\input{generated/reqdefs-SP-PDS}
\input{generated/reqdefs-DP-PDS}
\input{generated/reqdefs-SP-DAQ}
\input{generated/reqdefs-DP-DAQ}
\input{generated/reqdefs-SP-CISC}
\input{generated/reqdefs-DP-CISC}
\input{generated/reqdefs-SP-ELEC}
\input{generated/reqdefs-DP-ELEC}
\input{generated/reqdefs-SP-CALIB}
\input{generated/reqdefs-DP-CALIB}
\input{generated/reqdefs-SP-INST}
\input{generated/reqdefs-DP-INST}


==> vol-physics/ch-summ-concl.tex <==
%\chapter{Summary and Conclusions -- Placeholder}
%\label{ch:summ-concl}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\section{Summary of scientific impact in evolving global landscape}
%\label{ch:summ-concl-global}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\section{Broader impacts}
%\label{ch:summ-concl-broad}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\section{Concluding remarks}
%\label{ch:summ-concl-rem}
